Bayesian Tensorized Neural Networks with Automatic Rank Selection

Tensor decomposition is an effective approach to compress over-parameterized neural networks and to enable their deployment on resource-constrained hardware platforms. However, directly applying tensor compression in the training process is a challenging task due to the difficulty of choosing a proper tensor rank. In order to achieve this goal, this paper proposes a Bayesian tensorized neural network. Our Bayesian method performs automatic model compression via an adaptive tensor rank determination. We also present approaches for posterior density calculation and maximum a posteriori (MAP) estimation for the end-to-end training of our tensorized neural network. We provide experimental validation on a fully connected neural network, a CNN and a residual neural network where our work produces $7.4\times$ to $137\times$ more compact neural networks directly from the training.

==> fig/cifar10conv.tex <==
\begin{table}[t]
  \caption{Simple Convolutional Model Results}
  \label{table: simple conv}
  \centering
  \begin{tabular}{lllll}
    Model & SVGD Param $\#$ & Log-Likelihood & MAP Param $\#$  & MAP Accuracy \\
    \midrule
    BNN & 65,222,900 & -.512 & 1,304,458 & 88.6 \\
    BTNN-N & 7,026,600 & -.487 &   140,532  & 84.2  \\
    BTNN-RD & 3,148,350 & -.494 & 62,967 &  83.7 \\
    \bottomrule
  \end{tabular}
\end{table}

==> fig/cifar_basic_param_graph.tex <==

\begin{wrapfigure}{r}{2.6in}
%\begin{figure}
    \centering
    \includegraphics[width =.5\textwidth]{fig/cifar_basic}
    \caption{Parameter number for each convolutional and fully-connected layer of each model. Compression ratio between standard and BTNN shown. Layer 1 is identical for all models and omitted. The y-axis is a log-scale.}
    \label{fig: cifar_basic_param_graph}
    \vspace{-1in}
\end{wrapfigure}

==> fig/tt_graphical_model.tex <==
\begin{tikzpicture}[
align = flush center,
font = \small]
\matrix [
    matrix of nodes,
    column sep = 0.5em,
    row sep = 1.3em, 
    draw, dashed,
    nodes = {solid},
    ] (m)
{  
|[empty]| &|[empty]|$\alpha_{1}$ & |[empty]|$a_\lambda$ & |[empty]|  $b_\lambda$ & |[empty]|$\alpha_{2}$ & |[empty]|$a_\lambda$ & |[empty]|  $b_\lambda$ & |[empty]|$\alpha_{3}$ & |[empty]|$a_\lambda$ & |[empty]|  $b_\lambda$ & \\%end row 1
  |[empty]| &|[data]|$\psi_1$  &|[data]|$\lambda_1$ & |[empty]|  &|[data]|$\psi_2$  &|[data]|$\lambda_2$ &  |[empty]| & |[data]|$\psi_3$  &|[data]|$\lambda_3$ &  |[empty]|&|[empty]|$a_\tau$ & |[empty]|& |[empty]|$b_\tau$ & \\%end row 2
  |[data]|$\ten{G}_1$ &  |[empty]| & |[empty]| & |[data]|$\ten{G}_2$ & |[empty]| & |[empty]| &|[data]|$\ten{G}_3$ &  |[empty]| & |[empty]|& |[data]|$\ten{G}_4$ & |[empty]| & |[data]|$\tau$\\%end row 3
|[empty]| &  |[empty]| & |[empty]| & |[empty]| &  |[empty]| &|[data]|$\{x_i,y_i\}$ & |[empty]| & |[empty]|& |[empty]| & |[empty]|\\[.7em]
};
%from alpha_1, lambda
\draw[->](m-1-2) to (m-2-2);
\draw[->](m-1-3) to (m-2-3);
\draw[->](m-1-4) to (m-2-3);

%from alpha_2, lambda
\draw[->](m-1-5) to (m-2-5);
\draw[->](m-1-6) to (m-2-6);
\draw[->](m-1-7) to (m-2-6);

%from alpha_2, lambda
\draw[->](m-1-8) to (m-2-8);
\draw[->](m-1-9) to (m-2-9);
\draw[->](m-1-10) to (m-2-9);


%from psi_1
\draw[->](m-2-2) to (m-3-1);
\draw[->](m-2-2) to (m-3-4);

%from lambda_1
\draw[->](m-2-3) to (m-3-1);
\draw[->](m-2-3) to (m-3-4);

%from psi_2
\draw[->](m-2-5) to (m-3-4);
\draw[->](m-2-5) to (m-3-7);
%\draw[->](m-2-2) to (m-3-4);

%from lambda_2
\draw[->](m-2-6) to (m-3-4);
\draw[->](m-2-6) to (m-3-7);
%from psi_3
\draw[->](m-2-8) to (m-3-7);
\draw[->](m-2-8) to (m-3-10);

%from lambda_3
\draw[->](m-2-9) to (m-3-7);
\draw[->](m-2-9) to (m-3-10);

\draw[->](m-2-11) to (m-3-12);
\draw[->](m-2-13) to (m-3-12);

%to data
\draw[->](m-3-1) to (m-4-6);
\draw[->](m-3-4) to (m-4-6);
\draw[->](m-3-7) to (m-4-6);
\draw[->](m-3-10) to (m-4-6); 
\draw[->](m-3-12) to (m-4-6);
\end{tikzpicture}


\begin{figure}[t]
\label{fig:graphical model}
  \resizebox{\textwidth}{!}{
  \input{fig/tt_graphical_model.tex}
    }
 \caption{Elements of $\ten{G}_k$ and $\ten{G}_{k-1}$ controlled by $\boldsymbol\lambda^{(k)}$. Elements controlled by a single entry $\boldsymbol\lambda^{(k)}_l$ are grouped by color. Best viewed in color.**REPLACE WITH TENSOR PICTURE AND DEPTH**}
\end{figure}
